Planning and Synthesis Under Assumptions

In Reasoning about Action and Planning, one synthesizes the agent plan by taking advantage of the assumption on how the environment works (that is, one exploits the environment's effects, its fairness, its trajectory constraints). In this paper we study this form of synthesis in detail. We consider assumptions as constraints on the possible strategies that the environment can have in order to respond to the agent's actions. Such constraints may be given in the form of a planning domain (or action theory), as linear-time formulas over infinite or finite runs, or as a combination of the two. We argue though that not all assumption specifications are meaningful: they need to be consistent, which means that there must exist an environment strategy fulfilling the assumption in spite of the agent actions. For such assumptions, we study how to do synthesis/planning for agent goals, ranging from a classical reachability to goal on traces specified in \LTL and \LTLf/\LDLf, characterizing the problem both mathematically and algorithmically.

==> 5-solvingSUA.tex <==

In this section we report the complexity solving synthesis under assumptions for \LTL and \NBW.
\begin{theorem}\label{thm:solving:SUA}
\begin{enumerate} 
\item  \LTL synthesis under assumptions is $2$\exptime-complete.
\item \NBW synthesis under assumptions is \exptime-complete.
\end{enumerate}
\end{theorem}

\begin{proof}
The upper bounds follows from Theorem~\ref{thm:det} and Theorem~\ref{thm:synthesis}.
For the lower bound note that the problem of realizing $\gamma$ (known to be $2$\exptime-hard if $\gamma$ is given in \LTL and \exptime-hard if $\gamma$ is given by an \NBW, see Theorem~\ref{thm:synthesis}) is equivalent to the problem of realizing $\gamma$ under assumptions $\Omega \doteq Str_\env$. 
Now note that $\Omega$ is definable in \LTL and by \NBW. \srcomment{minor issue: statement of lower bounds for classic synthesis does not assume satisfiable $\gamma$}
\end{proof}


